A Novel Approach to Generate Correctly Rounded Math Libraries for New Floating Point Representations

Given the importance of floating-point~(FP) performance in numerous domains, several new variants of FP and its alternatives have been proposed (e.g., Bfloat16, TensorFloat32, and Posits). These representations do not have correctly rounded math libraries. Further, the use of existing FP libraries for these new representations can produce incorrect results. This paper proposes a novel approach for generating polynomial approximations that can be used to implement correctly rounded math libraries. Existing methods generate polynomials that approximate the real value of an elementary function $f(x)$ and produce wrong results due to approximation errors and rounding errors in the implementation. In contrast, our approach generates polynomials that approximate the correctly rounded value of $f(x)$ (i.e., the value of $f(x)$ rounded to the target representation). It provides more margin to identify efficient polynomials that produce correctly rounded results for all inputs. We frame the problem of generating efficient polynomials that produce correctly rounded results as a linear programming problem. Our approach guarantees that we produce the correct result even with range reduction techniques. Using our approach, we have developed correctly rounded, yet faster, implementations of elementary functions for multiple target representations.

==> figures/alg.calculatelambda.tex <==
\begin{figure}
\small
\begin{algorithm}[H]
\DontPrintSemicolon
\SetKwFunction{FMain}{Main}
\SetKwFunction{FCalculateLp}{Calculate$L'$}
\SetKwFunction{FCalculateLambda}{Calculate$\Lambda$}
\SetKwFunction{FGeneratePoly}{GeneratePoly}
\SetKwFunction{FAdjLower}{AdjLower}
\SetKwFunction{FAdjHigher}{AdjHigher}
\SetKwFunction{FHex}{Hex}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FCalculateLambda{$L'$}}{
    $X' \leftarrow \emptyset$\;
    $\Lambda \leftarrow \emptyset$\;
    \ForEach{$(\chi_{x_i}', I_{x_i}') \in L'$}{
        \If{$\chi_{x_i}' \notin X'$} {
            $X' \leftarrow X' \cup \{\chi_{x_i}'\}$
        }
    }
    
    \ForEach{$\chi_i \in X'$} {
        $\Omega_i \leftarrow \emptyset$
        \ForEach{$(\chi_{x_j}', I_{x_j}') \in L'$} {
            \If{$\chi_i = \chi_{x_j}'$} {
                $\Omega_i \leftarrow \Omega_i \cup \{I_{x_j}'\}$
            }
        }
        $\Psi_i \leftarrow \bigcap_{I_{x_j}' \in \Omega_i} I_{x_j}'$\;
        \lIf{$\Psi_i = \emptyset$} {
            \Return{$\emptyset$}
        }
        $\Lambda \leftarrow \Lambda \cup \{(\chi_i, \Psi_i)\}$\;
    }
    \Return{$\Lambda$}\;
    
  }
\end{algorithm}
\caption{The function \texttt{Calculate}$\Lambda$ combines multiple constraints, \ie $(\chi_{x_i}', I_{x_i}'), (\chi_{x_j}', I_{x_j}') \in L'$ where $\chi_{x_i}' = \chi_{x_j}'$, into a single constraint and creates a final list of constraints $\Lambda$ for $P_{\mathbb{H}}$.}
\label{algo:calculatelambda}
\end{figure}

==> sections/sec.approach.tex <==
\section{Approach}
To create a correctly rounded approximation function $C_{f, \mathbb{T}}(x)$, we formulate the problem of creating the implementation into (1) identifying a list of constraints $\Lambda$ that must be satisfied by $P_{\mathbb{H}}(x)$, \ie for all $(\chi_i, \Psi_i) \in \Lambda$, $P_{\mathbb{H}}(\chi_i) \in \Psi_i$, and (2) generate a $P_{\mathbb{H}}(x)$ that satisfies $\Lambda$. Thus, the major challenge in our approach is to correctly identify all $(\chi_i, \Psi_i) \in \Lambda$ such that if $P_{\mathbb{H}}(\chi_i) \in \Psi_i$, then $C_{f, \mathbb{T}}(x_i) = RN_{\mathbb{T}}(f(x_i))$ for all $x_i \in \mathbb{T}$ such that $\chi_i = RR_{\mathbb{H}}(x_i)$.

To accomplish this goal, we use a 4-step approach to generate  $P_{\mathbb{H}}(x)$:
\begin{enumerate}
    \item For every non-special-case input $x_i \in [a, b] \subseteq \mathbb{T}$ where $[a, b]$ is the domain of the function $f(x)$, we compute $y_i = RN_{\mathbb{T}}(f(x_i))$ using arbitrary precision arithmetic and use $y_i$ to identify $I_{x_i}$ such that for all $v \in I_{x_i}$, $RN_{\mathbb{T}}(f(x_i)) = y_i$. The pair, $(x_i, I_{x_i})$, defines a constraint on $A_{f, \mathbb{H}}$, \ie we must guarantee $A_{f, \mathbb{H}}(x_i) \in I_{x_i}$ to satisfy Theorem ~\ref{thm:approx_interval}. This step produces a list, $L$, that contains the list of constraints $(x_i, I_{x_i})$ for all $x_i$.
    
    \item For every constraint $(x_i, I_{x_i}) \in L$, we reduce the constraint to produce $(\chi_{x_i}', I_{x_i}')$, such that
    \[
    P_{\mathbb{H}}(\chi_{x_i}') \in I_{x_i}' \implies A_{f, \mathbb{H}}(x_i) = OC_{\mathbb{T}}(P_{\mathbb{H}}(RR_{\mathbb{T}}(x_i)) \in I_{x_i}
    \]
    where $\chi_{x_i}' = RR_{\mathbb{H}}(x_i)$. 
    %
    This step produces a list $L'$ containing the constraints $(\chi_{x_i}', I_{x_i}')$. $L'$ is a list of constraints that $P_{\mathbb{H}}$ must satisfy to ensure that $A_{f, \mathbb{H}}(x_i) \in I_{x_i}$.
    
    \item Depending on the range reduction function, there can be multiple constraints in $L'$ where $\chi_{x_i}'$ have the same value. More specifically, it is possible that there exists multiple  constraints, $(\chi_{x_1}', I_1'), (\chi_{x_2}', I_2'), \dots (\chi_{x_n}', I_n') \in L'$ such that $\chi_{x_1}' = \chi_{x_1}' = \dots \chi_{x_n}'$ and for all $1 \leq i, j \leq n$, $x_i \neq x_j$. In this case, we combine these constraints to a single constraint, $(\chi_i, \Psi_i)$. This step produces a list, $\Lambda$ that contains the constraints, $(\chi_i, \Psi_i)$ such that if $P_{\mathbb{H}}$ satisfies $\Lambda$, then it also satisfies $L'$.
    
    \item Finally, we generate the polynomial approximation $P_{\mathbb{H}}(x)$ that satisfies all constraints specified in $\Lambda$ using an arbitrary precision LP solver.
\end{enumerate}

In the remainder of this section, we describe our approach on each of the steps in more detail and the challenges we face in each step. The full implementation detail of each step will be described in Section ~\ref{sec:implementation}.

\subsection{Step 1: Identifying the bounds for $A_{f, \mathbb{H}}$}
\label{sec:approach:l}
Given a function we want to approximate, $f(x)$, let us define a set of values $X$ such that $X = [a, b] \cap \mathbb{T} - SP$ where $[a, b]$ is the domain of $f(x)$ and $SP$ is the set of special case inputs. To ensure a correctly rounded approximation $C_{f, \mathbb{T}}(x)$, our first step is to identify an interval $I_{x_i} \subseteq \mathbb{H}$ for each input $x_i \in X$ that satisfies the condition for the following theorem:

\begin{theorem}{}
\label{thm:ind_interval}
Given an input $x_i \in X$, define a non-empty interval $I_{x_i} \subseteq \mathbb{H}$ such that for all $v \in I_{x_i}$, $RN_{\mathbb{T}}(v) = RN_{\mathbb{T}}(f(x_i))$. If $A_{f, \mathbb{H}}(x_i) \in I_{x_i}$, then $RN_{\mathbb{T}}(A_{f, \mathbb{H}}(x_i)) = RN_{\mathbb{T}}(f(x_i))$.
\end{theorem}
If Theorem ~\ref{thm:ind_interval} holds for all $x_i \in X$, then Theorem ~\ref{thm:approx_interval} holds. Thus, our goal in this step is to identify the interval $I_{x_i}$ that holds Theorem ~\ref{thm:ind_interval}.

Identifying $I_{x_i}$ depends on the specifications of $\mathbb{T}$ and $\mathbb{H}$. For commonly used limited precision representations discussed in Section ~\ref{sec:finiteprecision}, $I_{x_i}$ can be computed using the rounding rule: Let $y_i = RN_{\mathbb{T}}(f(x_i))$. Then, $I_{x_i}$ is an interval around $y_i$ where all values $v \in I_{x_i}$ rounds to $y_i$. More specifically, define two values $b_l, b_u \in \mathbb{B}$ that are adjacent to $y_i$ and $b_l < y_i < b_u$. Then, based on the rounding rule (RNE), all real values $v \in (lb, ub) = (\frac{b_l + y_u}{2}, \frac{y_i + b_u}{2})$ has the property $RN_{\mathbb{B}}(v) = y_i$, since $y_i$ is the closest value in $\mathbb{T}$. Moreover, if the bit-string representation of $y_i$ is even when interpreted as an unsigned integer, then the interval can be widened to $[lb, ub]$.

Without the loss of generality, let $(lb, ub)$ be the interval where all real values $v \in (lb, ub)$ rounds to $y_i$. Then, we can identify two values $l_i, h_i \in \mathbb{H}$ that satisfies $l_i = min \{v \mid v \in \mathbb{D}, \: v > lb\}$, $h_i = max \{v \mid v \in \mathbb{H}, \: v < ub \}$, and $l_i \leq h_i$. This is possible because $lb, ub \in \mathbb{H}$  and $lb < y_i < ub$ if $\mathbb{H}$ has at least 1 more precision bit than $\mathbb{T}$. Finally, interval $I_{x_i} = [l_i, h_i]$ satisfies Theorem \ref{thm:ind_interval}.

\textbf{Illustration.}
Consider the running example used in Section ~\ref{sec:overview} where $x_1 = 1.8671875$ and $y_1 = RN_{\mathbb{B}}(log_{10}(x_1)) = 0.271484375$. The two adjacent bfloat values of $y_1$ are $b_l = 0.26953125$ and $b_u = 0.2734375$. Because the bit-string representation of $y_1$ is odd when interpreted as unsigned integer (\texttt{0x3e8b}), all real values in the interval $(0.2705078125, 
0.2724609375)$ rounds to $y_1$ when rounded to a bfloat value. Then, our interval $I_{x_1} = [l_1, h_1]$ where
\begin{align}
    &l_1 = 0.270507812500000055511151231257827021181583404541015625 \nonumber \\ 
& h_1 = 0.272460937499999944488848768742172978818416595458984375 \nonumber
\end{align}

At the end of step 1, we produce a list $L$ that contains the constraints, $(x_i, I_{x_i})$ for all $x_i \in X$ where $I_{x_i}$ satisfies Theorem ~\ref{thm:ind_interval} for each $x_i$.

\subsection{Step 2: Identifying the bounds for $P_{\mathbb{H}}$}
\label{sec:approach:lp}
In a typical approximation of a transcendental function $f(x)$, $A_{f, \mathbb{H}}(x)$ performs range reduction on the input $x_i$, \ie $\chi_{x_i}' = RR_{\mathbb{H}}(x_i)$ and also output compensation on the output of $y_i' = P_{\mathbb{H}}(\chi_{x_i}')$, \ie $y_i = OC_{\mathbb{H}}(y_i', x_i)$. Therefore, for $A_{f, \mathbb{H}}$ to satisfy a constraint $(x_i, I_{x_i}) \in L$, we must put a constraint on the output of $y_i' = P_{\mathbb{H}}(\chi_{x_i}')$ such that $OC_{\mathbb{H}}(y_i', x_i) \in I_{x_i}$.

\begin{theorem}{}
\label{thm:p_bound}
Define an input reduction function $RR_{\mathbb{H}}(x)$ and the corresponding output compensation function $OC_{\mathbb{H}}(y', x)$ for $A_{f, \mathbb{H}}(x)$. Let $(x_i, I_{x_i})$ be a constraint for $A_{f, \mathbb{H}}$ that satisfies Theorem ~\ref{thm:ind_interval} for $x_i$ and  $I_{x_i}' \in \mathbb{H}$ be an interval where for all $v \in I_{x_i}'$, $OC_{\mathbb{H}}(v, x_i) \in I_{x_i}$. If $P_{\mathbb{H}}(\chi_{x_i}') \in I_{x_i}'$ where $\chi_{x_i}' = RR_{\mathbb{H}}(x_i)$, then $A_{f, \mathbb{H}}(x_i) = OC_{\mathbb{H}}(P_{\mathbb{H}}(RR_{\mathbb{H}}(x_i))), x_i) \in I_{x_i}$.
\end{theorem}

More intuitively, for each constraint $(x_i, I_{x_i}) \in L$, we're looking for an interval $I_{x_i}'$ such that if $y_i' \in I_{x_i}'$, then $OC_{\mathbb{H}}(y_i', x_i) \in I_{x_i}$. Then the pair $(\chi_{x_i}', I_{x_i}')$ defines a constraint on the output of $P_{\mathbb{H}}(\chi_{x_i}')$, \ie $P_{\mathbb{H}}(\chi_{x_i}') \in I_{x_i}'$.

Observe that in the context of computing the constraint $(\chi_{x_i}, I_{x_i}')$ on the polynomial $P_{\mathbb{H}}(x)$ that satisfies the Theorem ~\ref{thm:p_bound}, the output compensation function $OC_{\mathbb{H}}(y', x_i)$ can be interpreted as a function in terms of $y'$, \ie the value of $x_i$ is fixed: $OC_{\mathbb{H}}(y', x_i) = OC_{\mathbb{H}, x_i}(y')$. Thus, $I_{x_i}'$ is the input domain of $OC_{\mathbb{H}, x_i}(y')$ that satisfies for all $y_i' \in I_{x_i}'$, $OC_{\mathbb{H}, x_i}(y') \in I_{x_i}$ where $I_{x_i}$ is the output range of $OC_{\mathbb{H}, x_i}(y')$. Our goal is to identify the input domain $I_{x_i}'$.

For an arbitrary function $OC_{\mathbb{H}, x_i}(y')$, there is no general method to compute the input domain $I_{x_i}'$ that satisfies for all $v \in I_{x_i}'$, $OC_{\mathbb{H}, x_i}(v) \in I_{x_i}$. However, we found that the most commonly used range reduction functions for approximating transcendental functions have specific properties that allows us to properly identify $I_{x_i}'$. More specifically, the mathematical function that $OC_{\mathbb{H}, x_i}(y_i')$ implements (or in other words, the output compensation function evaluated in real number arithmetic, $OC_{\mathbb{R}, x_i}(y_i') = OC_{x_i}(y_i')$) typically has all of the following properties:
\begin{enumerate}
    \item $OC_{\mathbb{R}, x_i}(y')$ is a smooth, continuous, and bijective function for the output range of $I_{x_i}$.
    \item $OC_{\mathbb{R}, x_i}(y')$ is a strictly increasing or decreasing function for the output range of $I_{x_i}$.
    \item There exists an inverse function, $OC_{\mathbb{R}, x_i}^{-1}(y)$ for the output range of $I_{x_i}$ such that $v = OC_{\mathbb{R}, x_i}(OC_{\mathbb{R}, x_i}^{-1}(v))$ for all $v \in I_{x_i}$.
\end{enumerate}
For example, the output compensation function in Equation ~\eqref{eq:rr_ex} holds all of the above properties for all input domain. Even in rare cases where we encountered an output compensation function that does not have the above properties for all output range of $I_{x_i}$, \ie $OC_{\mathbb{R}, x_i}(y') = \frac{1}{y'}$ for $y'$ near $0$, inputs that induces $y' = 0$ can be treated as special case and be excluded from $X$. For the instances where the above properties hold, the following theorem also holds:
\begin{theorem}{}
\label{thm:inverse_real}
Let $OC_{\mathbb{R}, x_i}(y')$ have the properties explained above for the output range $I_{x_i} = [l_i, h_i]$. Define an interval $\iota_{x_i} = [\alpha, \beta]$ if  $OC_{\mathbb{R}, x_i}(y')$ is an increasing function or $\iota_{x_i} = [\beta, \alpha]$ if it's a decreasing function where $\alpha = OC_{\mathbb{R}, x_i}^{-1}(l_i)$ and $\beta = OC_{\mathbb{R}, x_i}^{-1}(h_i)$. Then, for all $y_i' \in \iota_{x_i}$, $OC_{\mathbb{R}, x_i}(y_i') \in I_{x_i}$.
\end{theorem}

In other words, the input domain $\iota_{x_i}$ can be identified by computing the inverse function $OC_{\mathbb{R}, x_i}^{-1}(y)$ for the upper and lower bounds of $I_{x_i}$. However, Theorem ~\ref{thm:inverse_real} does not strictly hold for $OC_{\mathbb{H}, x_i}(y')$, \ie the following proposition is not true.

\begin{proposition}{}
\label{prop:inverse_h}
Let $OC_{\mathbb{H}, x_i}(y')$ be the function that evaluates $OC_{\mathbb{R}, x_i}(y')$ in $\mathbb{H}$ and $OC_{\mathbb{H}, x_i}^{-1}(y)$ be the function that evaluates $OC_{\mathbb{R}, x_i}^{-1}(y)$ in $\mathbb{H}$ where $OC_{\mathbb{R}, x_i}(y')$ has the properties explained above for the output range $I_{x_i} = [l_i, h_i]$. Define an interval $\iota_{x_i}' = [\alpha, \beta]$ if $OC_{\mathbb{H}, x_i}(y)$ is an increasing function or $\iota_{x_i}' = [\beta, \alpha]$ if it's a decreasing function where $\alpha = OC_{\mathbb{H}, x_i}^{-1}(l_i)$ and $\beta = OC_{\mathbb{H}, x_i}^{-1}(h_i)$. If $y_i' \in \iota_{x_i}'$, then $OC_{\mathbb{H}, x_i}(y_i') \in I_{x_i}$.
\end{proposition}

Proposition ~\ref{prop:inverse_h} fails because there are computation error in the evaluation of $OC_{\mathbb{H}, x_i}(y')$ and $OC_{\mathbb{H}, x_i}^{-1}(y)$. The actual bound on $I_{x_i}'$ that satisfies Theorem ~\ref{thm:p_bound} may be smaller than $\iota_i$. \textbf{NOTE: I'm not sure if the following proposition should go into implementation section.} In our empirical evaluation, we have found that the following proposition has held true for all of our evaluation:
\begin{proposition}{}
\label{prop:inverse_h_reduced}
Let $OC_{\mathbb{H}, x_i}(y')$ be the function that evaluates $OC_{\mathbb{R}, x_i}(y')$ in $\mathbb{H}$ and $OC_{\mathbb{H}, x_i}^{-1}(y)$ be the function that evaluates $OC_{\mathbb{R}, x_i}^{-1}(y)$ in $\mathbb{H}$ where $OC_{\mathbb{R}, x_i}(y')$ has the properties explained above for the output range $I_{x_i} = [l_i, h_i]$. Define an interval $[\alpha, \beta]$ where $\alpha = OC_{\mathbb{H}, x_i}^{-1}(l_i)$ and $\beta = OC_{\mathbb{H}, x_i}^{-1}(h_i)$ if $OC_{\mathbb{H}, x_i}$ is an increasing function or vice versa if it is a decreasing function. Denote $I_{x_i}' = [l_i', h_i']$ where $l_i' = min\{v \in \mathbb{H} \mid \alpha \leq v \text{ and } OC_{\mathbb{H}, x_i}(v) \in I_{x_i} \}$ and $h_i' = max\{v \in \mathbb{H} \mid v \leq \beta \text{ and } OC_{\mathbb{H}, x_i}(v) \in I_{x_i} \}$. Then, for all $y_i' \in I_{x_i}'$,  $OC_{\mathbb{H}, x_i}(y_i') \in I_{x_i}$.
\end{proposition}
\textbf{Note: Maybe Proposition ~\ref{prop:sufficient_interval} is easier to understand? Proposition ~\ref{prop:inverse_h_reduced} is the literal translation from our implementation, but perhaps Proposition ~\ref{prop:sufficient_interval} can be used to explain it in simpler term. I am not sure.}

Abstractly speaking, Proposition ~\ref{prop:inverse_h_reduced}, if true, allows us to compute the domain $I_{x_i}'$ that satisfies Theorem ~\ref{thm:p_bound} by initially computing the interval $[\alpha, \beta]$ that closely approximates $I_{x_i}'$ using the $OC_{\mathbb{H}, x_i}^{-1}(y')$ and then refine $[\alpha, \beta]$ by reducing the bounds until the resulting interval $I_{x_i}'$ satisfies Theorem ~\ref{thm:p_bound}. At the end of this step, we produce a list $L'$ that contains $(\chi_{x_i}', I_{x_i}')$ for each constraint $(x_i, I_{x_i}) \in L$. $L'$ is a list of constraints for $P_{\mathbb{H}}$. We explain step 2 in more detail in Section ~\ref{sec:implementation}. 

\subsection{Step 3: Merging bounds in $L'$}
\label{sec:approach:lambda}
Depending on the function $f(x)$ and the choice of range reduction algorithm, $RR_{\mathbb{H}}(x)$ and $OC_{\mathbb{H}}(y', x)$, it is possible that there exists multiple constraints, $(\chi_{x_i}', I_{x_i}'), \dots, (\chi_{x_j}', I_{x_j}') \in L'$ such that $\chi_{x_i}' = \dots = \chi_{x_j}'$ but $x_i \neq \dots \neq \ x_j$. More specifically, if we define a set $\Gamma_{\chi_k} = \{(\chi_{x_i}', I_{x_i}') \in L' \mid \chi_{x_i}' = \chi_k \}$, it is possible that $|\Gamma_{\chi_k}| > 1$, where $|\Gamma_{\chi_k}|$ is the number of constraints in $\Gamma_{\chi_k}$.

Intuitively, $P_{\mathbb{H}}(\chi_k)$ has to satisfy all constraints in $|\Gamma_{\chi_k}|$ in order to guarantee that $OC_{\mathbb{H}}(P_{\mathbb{H}}(RR_{\mathbb{H}}(x_i)) \in I_{x_i}$ for all constraints $(x_i, I_{x_i}) \in L$ where $RR_{\mathbb{H}}(x_i) = \chi_k$. In other words, $\Gamma_{\chi_k}$ specifies the constraint,
\begin{align}
P_{\mathbb{H}}(\chi_k) \in \Psi_k = \bigcap_{(\chi_k, I_{x_i}') \in \Gamma_{\chi_k}} I_{x_i}' \nonumber
\end{align}
Thus, we merge the constraints in $\Gamma_{\chi_k}$ to a single constraint, $(\chi_k, \Psi_k)$. Likewise, for all other sets of constraints $\Gamma_{\chi_i} \subseteq L'$ that includes all constraints $(\chi_i', I_{x_j}') \in L'$ are merged to a new constraint, $(\chi_i, \Psi_i)$. These constraints are stored in a new list $\Lambda$ that bounds the output of $P_{\mathbb{H}}$.

\subsection{Step 4: Generating $P_{\mathbb{H}}(x)$ that satisfies $\Lambda$}
Once we identify the constraints $\Lambda$ for $P_{\mathbb{H}}(x)$, the final step in our approach is to generate a polynomial $P_{\mathbb{H}}(x)$ such that for all $(\chi_i, \Psi_i) \in \Lambda$, $P_{\mathbb{H}}(\chi_i) \in \Psi_i$. Observe that each constraint, $(\chi_i, \Psi_i)$ specifies a linear constraint on $P_{\mathbb{H}}(x)$, \ie if we define $\sigma_i$ and $\mu_i$ such that $\Psi_i = [\sigma_i, \mu_i]$, then it specifies a constraint,
\[
\sigma_i \leq c_0 + c_1 \chi_i + c_2 (\chi_i)^2 + ... + c_d (\chi_i)^d \leq \mu_i
\]
on a polynomial $P_{\mathbb{H}}$ with degree $d$, where $c_0, c_1, ..., c_d$ is the desired coefficients for $P_{\mathbb{H}}$.

Therefore, we can formulate the problem of finding $P_{\mathbb{H}}(x)$ that satisfies all constraints in $\Lambda$ as solving for the coefficients $(c_0, c_1, \dots, c_d) \in \mathbb{H}^{(d+1)}$ that satisfies the set of linear constraints,
\begin{align}
\begin{bmatrix}
\sigma_1 \\
\sigma_2 \\
\sigma_3 \\
\vdots \\
\sigma_{|\Lambda|}
\end{bmatrix}
\leq
\begin{bmatrix}
1 && \chi_1 && \dots && (\chi_1)^d \\
1 && \chi_2 && \dots && (\chi_2)^d \\
1 && \chi_3 && \dots && (\chi_3)^d \\
\vdots && \vdots && \ddots && \vdots \\
1 && \chi_{|\Lambda|} && \dots && (\chi_{|\Lambda|})^d
\end{bmatrix}
\begin{bmatrix}
c_0 \\
c_1 \\
c_2 \\
\vdots \\
c_d
\end{bmatrix}
\leq
\begin{bmatrix}
\mu_1 \\
\mu_2 \\
\mu_3 \\
\vdots \\
\mu_{|\Lambda|}
\end{bmatrix}
\label{eq:lineq}
\end{align}

when all operations in $P_{\mathbb{H}}(x)$ are performed in $\mathbb{H}$. If there exists a $(c_0, c_1, \dots, c_d) \in \mathbb{H}^{(d+1)}$ such that the evaluation of $P_{\mathbb{H}}(\chi_i) \in \Psi_i$ for all constraints $(\chi_i, \Psi_i) \in \Lambda$, then $A_{f, \mathbb{H}}(x) = OC_{\mathbb{H}}(P_{\mathbb{H}}(RR_{\mathbb{H}}(x)), x)$ satisfies all constraints in $L$ and $C_{f, \mathbb{T}}(x)$ produces the correctly rounded value for all $x \in \mathbb{T}$.

Equation ~\eqref{eq:lineq} can be solved using linear programming (LP) solvers. However, one challenge in using an LP solver to solve for Equation ~\eqref{eq:lineq} is that (1) many publicly available LP solvers experience numerical errors in its own computation and (2) even if the LP solver provides a solution without experiencing numerical errors, the solution provided by the LP solvers only guarantee that the evaluation of $P(\chi_i)$ computed in real numbers produces a value in the interval $\Psi_i$. It does not guarantee that the evaluation of $P_{\mathbb{H}}(\chi_i)$ computed in $\mathbb{H}$ produces a correctly value in the interval $\Psi_i$.

Thus, we propose a sound iterative algorithm which utilizes an arbitrary precision LP solver to solve for the coefficients, $(c_0, c_1, \dots, c_d) \in \mathbb{H}^{(d+1)}$, verify that the resulting $P_{\mathbb{H}}$ does indeed produce values that satisfies $\Lambda$, and if it does not, refines the constraints in $\Lambda$ by restricting $\Psi_i$ to a smaller interval and repeats the process. We describe this technique in more detail in Section ~\ref{sec:implementation:solver}. Our algorithm for generating $P_{\mathbb{H}}$ is sound, \ie if it produces a polynomial $P_{\mathbb{H}}$ then $P_{\mathbb{H}}$ definitely satisfies $\Lambda$, and is guaranteed to terminate if the underlying LP solver that it uses terminates.
